Generating Hypothetical Events for Abductive Inference

Abductive reasoning starts from some observations and aims at finding the most plausible explanation for these observations. To perform abduction, humans often make use of temporal and causal inferences, and knowledge about how some hypothetical situation can result in different outcomes. This work offers the first study of how such knowledge impacts the Abductive NLI task -- which consists in choosing the more likely explanation for given observations. We train a specialized language model LMI that is tasked to generate what could happen next from a hypothetical scenario that evolves from a given event. We then propose a multi-task model MTL to solve the Abductive NLI task, which predicts a plausible explanation by a) considering different possible events emerging from candidate hypotheses -- events generated by LMI -- and b) selecting the one that is most similar to the observed outcome. We show that our MTL model improves over prior vanilla pre-trained LMs fine-tuned on Abductive NLI. Our manual evaluation and analysis suggest that learning about possible next events from different hypothetical scenarios supports abductive inference.

==> results.tex <==
\begin{table}[t!]
\small
\centering
{
\scalebox{1.0}{
%\hline 
\begin{tabular}{@{}l@{~}c@{~~}c@{~~}}
\toprule
{\bf Model} & {\bf Dev Acc.(\%)} & {\bf Test Acc.(\%)} \\\midrule
\hline
\textbf{\cite{bhagavatula2019abductive}}\\ 
Majority (\textit{from dev set})$^\diamond$ &{50.8}\\
DistilBERT &{62.2} &{61.03}  \\
BERT (Large)$^\diamond$ &{--}& 68.9\pm{0.5} \\
MTL &{71.2}& {70.86} \\
\hline
RoBerta (base) &{71.2} &{71.13} \\
MTL &{73.81} &\textbf{72.67} \\
%Roberta (large) &{82.06} &{81.74} \\
%RoBerta (large) + Forward Inference &{----} &\textbf{----} \\
\hline 
\textit{Human Performance} &-& 91.4\\
%\cline{1-5}
\bottomrule
\end{tabular}}}
\caption{Abductive NLI (Excluding unpublished leaderboard submissions)}\label{tab:finetune}
\end{table}

\begin{table}[t!]
\centering
{
\begin{tabular}{@{}l@{~}c@{~}c@{~}c@{~}c@{~}c@{~}}
\toprule
{\bf Model} & {BLUE-4} & {METEOR} & {ROUGE-L} & {CIDEr} & {BERT$_{score}$}\\\midrule
GPT-2$^\diamond$ &{0.00} & {9.29} & {9.99} & {3.34} & {36.69}\\
O1-O2 only$^\star$ $^\diamond$ & {2.23} & {16.71} & {22.83} & {33.54} & {48.74} \\
COMeT-Txt+GPT2$^\star$ $^\diamond$ & {2.29} & {16.73} & 22.51 & 31.99 & 48.46\\
COMeT-Emb+GPT2$^\star$ $^\diamond$ & {3.03} & 17.66 & 22.93 & 32.00 & 48.52\\
Forward Inference & {0.78} & {15.08} & {19.21} & \textbf{20.49} & \textbf{50.2} \\
Forward Inference$^\star$ & {2.08} & \textbf{20.65} & \textbf{23.36} & \textit{56.84} & \textbf{51.22} \\\hline
Human-written$^\diamond$ & 8.25 & 26.71 & 30.40 & 53.56 & 53.30\\
\bottomrule
\end{tabular}}
\caption{Results on automatic metrics for our models (NLG). $^\star$ finetuned on $\mathcal{ART}$, $^\diamond$ \cite{bhagavatula2019abductive}}\label{tab:automaticeval}
\end{table}

\begin{table*}[t]
\centering
\small
\scalebox{1.0}{
\begin{tabular}{@{}p{4cm}p{4cm}p{3cm}p{3cm}}
\toprule
\textbf{Observation} & \textbf{Hypothesis} &\textbf{FI} & \textbf{CFI}\\\hline
\textit{Dotty was being very grumpy. She felt much better afterwards} & {Dotty ate something bad.} & {she got a bad stomach ache.} & {she started to feel sick.}  \\
{} & {\textbf{Dotty call some close friends to chat.}} & {they all agreed to meet at the park to play} & {they all tried to make her happy.} \\\hline
\textit{Priya decided to try a new restaurant.  Priya thought her food was delicious.
} & {\textbf{She ordered two shrimp dishes.}} & {priya ate her shrimp dish.} & {she was excited to try them out.} \\
{} & {The food that Priya ordered was microwaved and precooked.} & {priya was very happy with her new meal.} & {priya was disappointed in the quality of the food.} \\\hline
\textit{Jim got ready for his first date. Since then, she has ignored all of Jim's text messages.} & { \textbf{Jim's date wasn't attracted to him.}} & {Jim was disappointed.} & {He tried to get her number. She never responded to him.} \\
{} & {Jim went on the date and said he didn't like the girl.} & {The girl said she liked Jim} & {He told her that he didn't want to date her.} \\
\bottomrule
\end{tabular}
}
\caption{Example of Forward Inference.
%between pairs of argumentative units.
}
\label{tbl:examples}
\end{table*}



==> supplementary_material.tex <==
\section{Appendix}
\if false
\subsection{Baselines \& Hyperparameter}
\paragraph{$\alpha$NLI Task.} The baselines are as follows:
\begin{itemize}
    \item \textit{ESIM + ELMo} \cite{chen-etal-2017-enhanced} uses (a) ELMo to encode the observations and hypothesis, followed by (b) an attention layer, (c) a local inference layer, and (d) another bi-directional LSTM inference composition layer, and (e) a pooling operation, 
    \item \textit{Infersent} \cite{conneau-etal-2017-supervised} uses sentence encoding based on a
bi-directional LSTM architecture with max pooling.
    \item \textit{BERT} \cite{devlin-etal-2019-bert} is a LM trained with a masked-language modeling (MLM) and next sentence prediction objective. 
\end{itemize}
\paragraph{Our setup.} We used the following set of hyperparameters for our $\mathcal{MTL-FI}$: batch size: $8, 16$; epochs: \{$3, 5$\}; learning rate: \{$2e$-$5$, $5e$-$6$\}; For evaluation, we measure accuracy. We use Adam Optimizer, and dropout rate = $0.1$. We experimented on GPU size of $11$GB and $24$GB. Training is performed using cross-entropy loss. The loss function: $\mathcal{L}_{\alpha NLI}$ + $w*\mathcal{L}_{similarity}$; where $w$ is trainable parameter. During our experiment we initialize $w=1$. Interesting, after training the model we found w value varied from $0.85$ to $0.75$ showing the importance of our forward inference. The input format is depicted in Table \ref{tab:format}. 
\fi 







\begin{table*}[t!]
\centering
\small
\scalebox{1.0}{
\begin{tabular}{@{}p{6cm}p{4cm}p{5cm}}
\toprule
\textbf{Observation ($O$)} & \textbf{Hypothesis ($H_j$)} & \textbf{Generated Implications $O_{2}^{H_j}$}\\\hline
\textit{${O_1}$: Dotty was being very grumpy. ${O_2}$: She felt much better afterwards} & $H_1$: {Dotty ate something bad.} & $O_{2}^{H_1}$:{She started to feel sick.}  \\
{} & $H_2$:{\textbf{Dotty call some close friends to chat.}} & $O_{2}^{H_2}$: {They all tried to make her happy.} \\\hline
\textit{${O_1}$: Priya decided to try a new restaurant. ${O_2}$: Priya thought her food was delicious.
} & {$H_1$:\textbf{She ordered two shrimp dishes.}} & {$O_{1}^{H_2}$: She was excited to try them out.} \\
{} & {$H_2$: The food that priya ordered was microwaved and precooked.} & {$O_{2}^{H_2}$: Priya was disappointed in the quality of the food.} \\\hline
\textit{${O_1}$: Jim got ready for his first date. ${O_2}$: Since then, she has ignored all of Jim's text messages.} & { $H_1$: \textbf{ Jim's date wasn't attracted to him.}} & {$O_{1}^{H_2}$: He tried to get her number. She never responded to him.} \\
{} & {$H_2$: Jim went on the date and said he didn't like the girl.} & {$O_{2}^{H_2}$: He told her that he didn't want to date her.}\\\hline
\textit{${O_1}$: Cay had a crush on a boy in her class.	 ${O_2}$: He smiled at her after and said he liked her too!} & 
{$H_1$: \textbf{Cay sent a love note to the boy.}} & {$O_{1}^{H_2}$: The boy responded and said he liked Cay.} \\
{} & {$H_2$: She told him she did not like him.} & {$O_{2}^{H_2}$: The boy was very sad about it. }\\\hline
\textit{${O_1}$: Daniel wanted to buy a toy plane, but he didn't have any money. ${O_2}$: He bought his toy plane, and kept working so he could buy another!} & $H_1$: {\textbf{He opened a lemonade stand.}} & {$O_{1}^{H_2}$: He sold lemonade for a lot of money .} \\
{} & $H_2$: {Daniel stayed home and didn't want to buy a plane.} & {$O_{2}^{H_2}$: He decided he needed to get a part time job.}\\\hline
\textit{${O_1}$: Ali's mom enrolled her in a karate class. ${O_2}$: Ali was so embarrassed she didn't tell any of her friends.} & $H_1$: \textbf{Ali did not want to take karate.} & $O_{2}^{H_1}$: {She was afraid she would get hurt.}  \\
{} & {$H_2$: Ali did horribly in her last class.} & {$O_{2}^{H_2}$: Ali was so embarrassed. She tried to hide it from her parents.}\\
\bottomrule
\end{tabular}}\caption{Example of generated implications using  $\mathcal{FI}$ model.}
\label{tab:anli_example}
\end{table*}




